Transient Concepts in Streaming Graphs

Concept Drift (CD) occurs when a change in a hidden context can induce changes in a target concept. CD is a natural phenomenon in non-stationary settings such as data streams. Understanding, detection, and adaptation to CD in streaming data is (i) vital for effective and efficient analytics as reliable output depends on adaptation to fresh input, (ii) challenging as it requires efficient operations as well as effective performance evaluations, and (iii) impactful as it applies to a variety of use cases and is a crucial initial step for data management systems. Current works are mostly focused on passive CD detection as part of supervised adaptation, on independently generated data instances or graph snapshots, on target concepts as a function of data labels, on static data management, and on specific temporal order of data record. These methods do not always work. We revisit CD for the streaming graphs setting and introduce two first-of-its-kind frameworks SGDD and SGDP for streaming graph CD detection and prediction. Both frameworks discern the change of generative source. SGDD detects the CDs due to the changes of generative parameters with significant delays such that it is difficult to evaluate the performance, while SGDP predicts these CDs between 7374 to 0.19 milliseconds ahead of their occurrence, without accessing the payloads of data records.

==> tableOfnotations.tex <==
\begin{table}[!ht]
 \centering \resizebox{8.5cm}{!}{

    \begin{tabular}{p{2.9cm}p{10cm}}\hline
        
        Notation & Description \\ \hline
        
        $r_m=\langle p_m,\tau_m \rangle$ &  Streaming Graph Record (SGR) with index $m$ \\ 
        $p_m$ & Payload of $r_m$\\
        $\tau_m$& Generation timestamp of $r_m$\\
        $t_m$ & Arrival time of $r_m$\\ 
        $\Re=\langle r_1,r_2,... \rangle$ & Streaming graph\\
        $b$ & A burst\\
        $B$, $\bar{B}$, $maxB$ & Burst size, The average seen burst size, The maximum seen burst size \\
        %$V_i=\{v_i\}$, $V_j=\{v_j\}$ & Set of i-vertices, Set of j-vertices\\
        %$G_{W,t}$ &  A graph snapshot formed by window $W$ at time $t$ \\ 
        %$N(v)=\{n\mid e_{vn}\in E\}$ & One-hop neighbourhood of a vertex v\\
        %$N_j(v_i)$ & One-hop neighbours of an i-vertex $v_i$ called j-neighbours\\
        %$e_{vn}=(v,n,w_{vn})$ & A unipartite weighted edge between vertices $v$ and $n$ with weight $w_{vn}$\\
        %$e_{ij}=(v_i,v_j)$ & A bipartite edge between vertices $v_i$ and $v_j$\\
        
        %$\rtimes$ & Caterpillar\\
        %$\bowtie^{i_1,i_1}_{j_1,j_2}$, $\newbowtie$, $\newbowtie_v$ & Butterfly, Young butterfly,  Young butterfly mapped to vertex v\\
        %$\newbowtie$ & Young butterfly \\
        
        %\th & Structural pattern \\
        
        
        %$P(\newbowtie_v)=v$ & Projection function mapping a young butterfly to a unipartite vertex $v$\\ 
        %\bigcap(\newbowtie_u, \newbowtie_v)$ & Set of common vertices in two butterflies $\newbowtie_u$ and $\newbowtie_v$\\
        
        %$\Omega_v$, $\theta_v$  & Frequency of phase oscillator (vertex) $v$, Phase of phase oscillator (vertex) $v$ \\
        
        %$O=\langle O[1],\cdots,O[t] \rangle$ & Sequence of order parameter values\\
        
        %$\lambda$ & Drift detection threshold\\
        %S & Drift detection suffix size \\
        \hline
        
\end{tabular}}\caption{Notations used in the paper.} \label{tab:notations}
\normalsize
\end{table}
